Tighter Variational Bounds are Not Necessarily Better

We provide theoretical and empirical evidence that using tighter evidence lower bounds (ELBOs) can be detrimental to the process of learning an inference network by reducing the signal-to-noise ratio of the gradient estimator. Our results call into question common implicit assumptions that tighter ELBOs are better variational objectives for simultaneous model learning and inference amortization schemes. Based on our insights, we introduce three new algorithms: the partially importance weighted auto-encoder (PIWAE), the multiply importance weighted auto-encoder (MIWAE), and the combination importance weighted auto-encoder (CIWAE), each of which includes the standard importance weighted auto-encoder (IWAE) as a special case. We show that each can deliver improvements over IWAE, even when performance is measured by the IWAE target itself. Furthermore, our results suggest that PIWAE may be able to deliver simultaneous improvements in the training of both the inference and generative networks.

==> background.tex <==
% !Tex root=./main.tex

\section{Evidence Lower Bounds and the Importance Weighted Auto-Encoder}

More generally, as shown by~\cite{maddison2017filtering,anonymous2018auto-encoding}, one can express the bound
between a general \gls{ELBO} and the log marginal likelihood $\log Z_P$ given a non-negative unbiased estimator $\hat{Z}_P$
of $Z_P$ and a proposal distribution $Q(x)$ using
\begin{align}
\ELBO &= \int Q(x) \log \hat Z_P(x) \,\mathrm dx = \log Z_P - \KL{Q}{P},
\label{eqn:aesmc/bias/elbo3} \\
\text{where} \quad P(x) &= \frac{Q(x) \hat Z_P(x)}{Z_P} \label{eqn:aesmc/bias/P}
\end{align}
is a normalized target density.  We remind the reader that $\KL{Q}{P}\ge0$ with equality holding if and only if
$P=Q$.
In the case of \glspl{IWAE}, then taking $Q$ and $\hat Z_P$ as per \eqref{eq:background/q_is_z_is} yields
\begin{align}
\ELBO_{\text{IS}}(\theta, \phi, y) &= \log p_{\theta}(y) - \KL{Q_{\text{IS}}}{P_{\text{IS}}}, \text{ where } \label{eqn:aesmc/bias/elbo_is} \\
P_{\text{IS}}(x^{1:K}) &= \frac{1}{K} \sum_{k = 1}^K \left(q(x^1 \given y) \cdots q(x^{k - 1} \given y) p(x^k \given y) q(x^{k + 1} \given y) \cdots q(x^K \given y) \right),
\end{align}
while similar representations can be straightforwardly derived such as those of~\cite{le2017auto,maddison2017filtering,naesseth2017variational}.

Using these results,~\cite{anonymous2018auto-encoding} go on to show that
$Q_{\text{IS}}(x^{1:K}) = P_{\text{IS}}(x^{1:K})$ for all $x^{1:K}$ if and only if $q(x \given y) = p(x \given y)$ for all $x$.
Consequently, the global optimum of $\{\theta,\phi\}$ for the \gls{IWAE} (presuming the inference network is flexible enough to always be able to
match the generative network) is the same as that for the~\gls{VAE}.  This
suggests that the advantages of the \gls{IWAE} must
originate either from better efficiency in the training procedure or less susceptibility 
to local optima. We thus
argue that the difference in tightness between the two \glspl{ELBO} is an insufficient measure of the relative utility of the two
approaches and that one should instead look to the variance of the gradient estimates relative to their expected magnitude and
susceptibility to local optima to asses the relative merits of the different choices of \gls{ELBO}.  Though it is beyond the
scope of this work to properly assess the latter of these, investigation of the former will form the focus for the rest of the paper.

==> dir_proof.tex <==
% !Tex root=./main.tex

\section{Proof of Directional Convergence}
\label{sec:dirproof}

\dirproof*

\begin{proof}
Substituting~\eqref{eq:expt} into~\eqref{eq:dir_conv}, explicitly writing out
the denominator terms, and multiplying the numerator and denominators of the
first term by $2KZ^2$ gives
\begin{align*}
&\left\lVert \frac{-\nabla_{\phi} \text{Var}\left[w_{1,1}\right]
	+O\left(\frac{1}{K}\right)}
{\sqrt{\sum_{d=1}^{D} \left( \nabla_{\phi_d} \text{Var}\left[w_{1,1}\right]
	+O\left(\frac{1}{K}\right)\right)^2}}
-\frac{-\nabla_{\phi} \textnormal{Var}\left[w_{1,1}\right]}
{\sqrt{\sum_{d=1}^D \left(\nabla_{\phi_d} \textnormal{Var}\left[w_{1,1}\right]\right)^2}}
\right\rVert_2 \\
& 
= \left\lVert
\frac{
\left(-\nabla_{\phi} \text{Var}\left[w_{1,1}\right]\right)
\left(
\sqrt{\sum_{d=1}^D \left(\nabla_{\phi_d} \textnormal{Var}\left[w_{1,1}\right]\right)^2}
-\sqrt{\sum_{d=1}^{D} \left( \nabla_{\phi_d} \text{Var}\left[w_{1,1}\right]
	+O\left(\frac{1}{K}\right)\right)^2}\right)+O\left(\frac{1}{K}\right)
}
{
\sqrt{\sum_{d=1}^{D} \left( \nabla_{\phi_d} \text{Var}\left[w_{1,1}\right]
	+O\left(\frac{1}{K}\right)\right)^2}
\sqrt{\sum_{d=1}^D \left(\nabla_{\phi_d} \textnormal{Var}\left[w_{1,1}\right]\right)^2}	
}
\right\rVert
\end{align*}
\end{proof}
where $d$ indicates the dimension.

==> literature.tex <==
\section{Literature}
There has been extensive literature investigating how to make the ELBO a tighter bound to the log marginal likelihood by improving the variational posterior.
Broadly speaking, there are two approaches.

The first approach aims at making the \emph{learned} variational distribution more expressive, thereby allowing it to more closely approximate the true posterior \emph{when trained}.
This can be done by normalising flows \citep{rezende_variational_2015,kingma2016improving},
using auxiliary variables \citep{maaloe_auxiliary_2016} \citep{ranganath2016hierarchical}

The second approach improves upon the current variational distribution by algorithmic means. This can be done using particle methods including weighting \citep{burda2015importance} or resampling \citep{maddison2017filtering}\citep{le2017auto}. Alternatively, Markov Chain Monte Carlo can be used in latent space \citep{salimans_markov_2015}.
Another possibility is to use a different divergence measure as done in \citep{li2016renyi}.


To fit in:

Perturbative Black Box Variational Inference:
\citep{bamler_perturbative_2017}

Ladder VAEs:
\citep{so_nderby_ladder_2016}
This is weird but probably part of the first approach.

Variational Gaussian Process
\citep{tran_variational_2015}
Also weird but probably also part of first approach.

Christian Naesseth
\citep{naesseth2017variational}


==> piwae.tex <==
% !Tex root=main.tex

\section{The Partially Importance-Weighted Auto-Encoder}
\label{sec:piwae}

We have provided theoretical and empirical evidence that using a
lower $K$ is beneficial to calculating gradients of inference network,  while a higher $K$
is beneficial for the generative network.  From this it is natural to conclude
that one should use a different target for each network.  To this end, we introduce
the partially importance-weighted auto-encoder (\gls{PIWAE}), which for a given budget $T=KM$
sets $K=1$, $M=T$ for the inference network updates as per the \gls{VAE} and 
$K=T$, $M=1$ for the generative network updates as per the \gls{IWAE}.  Using
the general form of our estimator as per~\eqref{eq:grad-est}, the same importance
weights can be used for calculating both targets, thereby requiring only minimal
algorithmic changes to the \gls{IWAE}.  Namely, the gradient update algorithm for
\gls{PIWAE} is as follows.

\todo[inline]{Add algorithm block}


